InteractionBench: A Real-Time Interaction Benchmark for Streaming Video Systems

A video assistant must speak when its instruction warrants a response and stay silent otherwise. We introduce a benchmark that evaluates this decision for the complete system of model, memory, and response controller. InteractionBench covers query responses, event triggers, and ongoing updates in 1,060 interactions over 812 videos, with 69 negative streams and 53 suites that pair counted events with look-alike near misses. It scores content accuracy, timing accuracy, and silence compliance on the video clock. Timely speech costs silence across systems. Polled Qwen3-VL-8B reaches 77.8 timing accuracy but 10.9 silence compliance. A native real-time interaction system reaches 29.2 silence compliance at 66.8 timing accuracy, yet emits on 89.9% of negative streams. No open-weight system clears a third of the near-miss suites. Fewer replies help only when chosen, as random deletion merely trades timing for silence. Offline scores miss these failures and mispredict online behavior. Adding restraint is costly, as the native system's controller adds little by itself and agentic systems add it only at about 30 s per poll.

==> packages.tex <==
\RequirePackage{amsmath}
\RequirePackage{amsthm}
\RequirePackage{amssymb}
\RequirePackage{mathtools} %
\RequirePackage{bm} %
\RequirePackage{mathpazo}

\RequirePackage{microtype}
\RequirePackage{anyfontsize}
\RequirePackage{titlesec}
\RequirePackage{tocloft}
\RequirePackage[defaultsans]{lato} %

\RequirePackage{xcolor}
\RequirePackage{colortbl}
\definecolor{gblue}{HTML}{1A73E8} %
\definecolor{gred}{HTML}{D93025} %
\definecolor{gyellow}{HTML}{E37400} %
\definecolor{ggreen}{HTML}{1E8E3E} %
\definecolor{gpurple}{HTML}{9334E6} %
\definecolor{ggrey}{HTML}{5F6368} %
\colorlet{linkcol}{gblue}

\RequirePackage{graphicx}
\RequirePackage{svg} %
\RequirePackage{wrapfig}
\RequirePackage{adjustbox}
\RequirePackage{tikz} %

\RequirePackage[labelsep=colon]{caption}
\RequirePackage{subcaption} %

\RequirePackage{booktabs}
\RequirePackage{multirow}
\RequirePackage{tabularx}
\RequirePackage{makecell}

\RequirePackage{geometry}
\RequirePackage{fancyhdr}
\RequirePackage{authblk}
\RequirePackage{enumitem}
\RequirePackage{tcolorbox}

\RequirePackage{verbatim}
\RequirePackage{pifont}

\RequirePackage[ruled,vlined,linesnumbered]{algorithm2e}
\RequirePackage{minted} %

\RequirePackage[numbers,sort&compress]{natbib}

\RequirePackage[colorlinks=true,allcolors=linkcol]{hyperref}
\RequirePackage[capitalize,noabbrev]{cleveref} %

